Quantifying the Value of Revert Protection

Revert protection is a feature provided by some blockchain platforms that prevents users from incurring fees for failed transactions. We study the economic implications and benefits of revert protection in the context of priority gas auctions and maximal extractable value. We develop a model in which searchers bid for a top-of-block arbitrage opportunity under varying degrees of revert protection. This model applies to a broad range of settings, including bundle auctions on L1s and priority ordering sequencing rules on L2s. We quantify, in closed form, how revert protection improves equilibrium auction revenue, market efficiency, and blockspace efficiency.

==> archived-versions/0-nextsteps.tex <==
\section*{Next Steps}

Outline:
\begin{enumerate}
    \item Intro / lit review
    \begin{itemize}
        \item general discussion of pros and cons of revert protection (e.g., it is generally acknowledged as good, but has the downside of needing to simulate the block), more of an issue now with centralized sequencers in L2s
        \item contributions
        \item literature review
    \end{itemize}
    \item Model: \done
    \begin{itemize}
        \item define $V$, $N$, $b$, $g$, $r_1$, $r_2$ \done
        \item assumption: bidding does not impact base fee \done
        \item footnote to differentiate for existing auction settings (minimum base fee to bid, partial refunds, differential refund between $g$ and $b$) \done
        \item example: full revert protection $r_1=r_2=0$ (e.g., MEV boost) \done
        \item example: no revert protection $r_1=r_2> 0$ (e.g., mainnet) \done
        \item example: application level priority taxes $r_1>0, r_2 = 0$ \done
        \item define strategy space: $(\text{whether to participate},\text{how much to bid})$ \done
        \item give game payouts \done
    \end{itemize}
    \item Equilibrium Analysis
    \begin{itemize}
    \item theorem: no pure strategy equilibrium (even when non-symmetric) when $r > 0$ ($r_1$ vs. $r_2$) \done
    \item define symmetric randomized strategies: $(p,F(\cdot))$ \done
    \item give expected payoffs \done \textcolor{blue}{(in model section)}
    \item theorem: randomized symmetric equilibrium in general case \done
    \item possible theorem: equilibrium we find is unique \textcolor{blue}{(probably not true)}
    \item corollary: special case when $r_1=r_2=0$ is pure strategy to bid full value \textcolor{blue}{(don't think this follows from the symmetric mixed equilibrium, put as separate theorem)}
    \item discussion of impact of parameters on $(p,F(\cdot))$ \done
    \end{itemize}
    \item Comparative Statics / Discussion \done
    \begin{itemize}
    \item each of the below should have a theorem or corollary with the formula, and directionality as a function of parameters
    \item NRP is worse, but we quantify how
    \item impact of RP on base fee and priority fee revenue
    \item impact of RP on social welfare / total fees
    \item expected blockspace consumption
    \end{itemize}
    \item Case Study: CEX-DEX arbitrage
    \begin{itemize}
    \item price dynamics, describe the DEX, arb trade, etc.
    \item performance metrics: price accuracy, LP losses, sequencer revenue, arb profits
    \item simulation results
    \end{itemize}
\end{enumerate}

Random Notes:
\begin{enumerate}
    \item switch to ACM FC format
    \item all proofs should be in the appendix
    \item I don't think we need to be formal about MEV taxes, e.g., how much mev taxes are collected, but we should discuss
    \item this is pedantic and fee free to ignore, but I feel the use of $a\cdot b$ and $a \times b$ is excessive and makes the equations longer and hard to read
\end{enumerate}



==> archived-versions/Z-fact-checks.tex <==
\section{Fact Checks}

\subsection{Equilibrium Quantities}

\begin{itemize}
    \item Entry and bidding strategies:
    \begin{gather*}
        p = \left(\frac{r_1g}{V-g+r_1g}\right)^{\frac{1}{N-1}} \\[0.25\baselineskip]
        F(b) = \frac{1}{1-p}\left(\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right)^{\frac{1}{N-1}}-p\right)
    \end{gather*}
    \item Limiting expected number of txs:
    \begin{gather*}
        \lim_{N\to\infty}N(1-p) = \log\left(\frac{V-g+r_1g}{r_1g}\right)
    \end{gather*}
    \item Limiting probability of at least one tx:
    \begin{gather*}
        \lim_{N\to\infty}(1-p^N) = \frac{V-g}{V-g+r_1g}
    \end{gather*}
\end{itemize}

\subsection{Compare Equilibrium}

In the model of Hillman and Samet (1987), the action space is $x\in\{0\}\cup[c,V]$ where $c$ is the minimum outlay. The equilibrium CDF is
\begin{gather*}
    F(x) = \begin{dcases}
        \left(\frac{c}{V}\right)^{\frac{1}{N-1}} & x \in [0,c) \\[0.25\baselineskip]
        \left(\frac{x}{V}\right)^{\frac{1}{N-1}} & x \geq [c,V].
    \end{dcases}
\end{gather*}
In our model, the action space is $b\in\{\textsf{no entry}\}\cup[0,V-g]$. Since entering the auction requires one to pay the base fee $g$, the \textit{effective bid} is $x=g+b$, which is used in Hillman and Samet (1987). The transformed action space in terms of effective bids is thus $x\in\{0\}\cup[g,V]$. As $p$ is the probability of ``effectively bidding'' zero, the CDF in terms of effective bids is given by
\begin{gather*}
    F(x)=\begin{dcases}
        p & x=[0,g) \\
        p+(1-p)\cdot F(b) & x\in[g,V].
    \end{dcases}
\end{gather*}
The model of Hillman and Samet (1987) is a special case of our model where $r_1=r_2=1$ and $c=g$. The equilibrium strategy under these parameters in our model is
\begin{gather*}
    p = \left(\frac{c}{V}\right)^{\frac{1}{N-1}} \\[0.25\baselineskip]
    F(b) = \frac{1}{1-\left(\frac{c}{V}\right)^{\frac{1}{N-1}}}\left(\left(\frac{c+b}{V}\right)^{\frac{1}{N-1}}-\left(\frac{c}{V}\right)^{\frac{1}{N-1}}\right)=\frac{(c+b)^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}{V^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}},
\end{gather*}
The CDF in terms of the effective bid $x$ when $x\in[0,c)$ is thus
\begin{align*}
    F(x) = p = \left(\frac{c}{V}\right)^{\frac{1}{N-1}}, 
\end{align*}
and when $x\in[c,V]$, it is
\begin{align*}
    F(x) &= p+(1-p)\cdot F(b) \\[0.25\baselineskip]
    &= \left(\frac{c}{V}\right)^{\frac{1}{N-1}}+\left(1-\left(\frac{c}{V}\right)^{\frac{1}{N-1}}\right)\left(\frac{(c+b)^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}{V^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}\right) \\[0.25\baselineskip]
    &= \left(\frac{c}{V}\right)^{\frac{1}{N-1}}+\left(1-\left(\frac{c}{V}\right)^{\frac{1}{N-1}}\right)\left(\frac{x^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}{V^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}\right) \\[0.25\baselineskip]
    &= \left(\frac{c}{V}\right)^{\frac{1}{N-1}}+\frac{x^{\frac{1}{N-1}}-c^{\frac{1}{N-1}}}{V^{\frac{1}{N-1}}} = \left(\frac{x}{V}\right)^{\frac{1}{N-1}}
\end{align*}
since $x=g+b$. Thus our model equilibrium in the special case of Hillman and Samet (1987) is consistent with their independent derivation. 

\subsection{Revenue Decomposition}

To derive the base gas fee revenue (henceforth called the entrance fee), let $X$ be a random variable for the number of agents that enter. Conditional on $X=k$ for $k\geq1$, note that the winner pays the full base fee $g$ while the $(k-1)$ losers pay the revert cost of $r_1g$. Then
\begin{align*}
    \mathbb{E}[\textsf{Entrance Fees}] &= \sum_{k=1}^N\mathbb{P}(X=k)\cdot(g+(k-1)r_1g) \\[0.25\baselineskip] 
    &= r_1g\sum_{k=1}^Nk\cdot\mathbb{P}(X=k)+(1-r_1)g\sum_{k=1}^K\mathbb{P}(X=k) \\[0.25\baselineskip]
    &= N(1-p)r_1g+(1-p^N)(1-r_1)g.
\end{align*}
Expected bidding fees then follow from linearity of expectation. Thus
\begin{gather*}
    \mathbb{E}[\textsf{Total Fees}] = (1-p^N)V \\
    \mathbb{E}[\textsf{Entrance Fees}] = (1-p^N)g+(N(1-p)-(1-p^N))r_1g \\
    \mathbb{E}[\textsf{Bidding Fees}] = (1-p^N)(V-g)-(N(1-p)-(1-p^N))r_1g.
\end{gather*}
\textcolor{blue}{Can also write expected bidding fees as
\begin{align*}
    \mathbb{E}[\textsf{Bidding Fees}] = \sum_{k=1}^N\mathbb{P}(X=k)\cdot(r_2k\cdot\mathbb{E}X+(1-r_2)\cdot\mathbb{E}X^k_{(1)})
\end{align*}
where $X^k_{(1)}$ is the maximum (largest order statistic) of $k$ i.i.d draws of $X\sim F$.}

\subsection{MEV Taxes}

Suppose that the revert penalty rate is $r$ and the MEV tax rate is $\tau$. Given the base gas fee $g$ and an arbitrageur's priority fee bid $\beta_i$, their payment is
\begin{align*}
    \textsf{Payment}_i = \begin{dcases}
        g+\beta_i(1+\tau) & \text{$i$ wins} \\
        rg+r\beta_i & \text{$i$ loses}.
    \end{dcases}
\end{align*}
Let $b_i=(1+\tau)\beta_i$, $r_1=r$, and $r_2=r/(1+\tau)$ for the current parameterization:
\begin{align*}
    \textsf{Payment}_i = \begin{dcases}
        g+b_i & \text{$i$ wins} \\
        r_1g+r_2b_i & \text{$i$ loses}.
    \end{dcases}
\end{align*}
The MEV tax collected is $\tau\beta_{(1)}=\tau b_{(1)}/(1+\tau)$ where $b_{(1)}$ is the highest bid, if at least one exists. Then
\begin{align*}
    \mathbb{E}[\textsf{MEV Tax}] = \frac{\tau}{1+\tau} \sum_{k=1}^n \mathbb{P}(N=k)\cdot \mathbb{E} X^k_{(1)}
\end{align*}
where $X^k_{(1)}$ is the maximum (largest order statistic) of $k$ i.i.d draws of $X\sim F$.

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> archived-versions/Z-new-mixed-strategy-analysis.tex <==
\section{Mixed Strategy Nash Equilibrium}

We analyze a mixed strategy Nash equilibrium where arbitrageurs randomize their bids over a range of possible values. Let \( p \) represent the probability that an arbitrageur abstains from bidding, and for those who bid, let \( F(b) \) be the cumulative distribution function (CDF) representing the probability that the bid is strictly less than \( b \).

\subsection{Expected Payoff from Bidding}

Suppose an arbitrageur bids \( b \). The payoff from bidding depends on whether the bid wins or loses:
\begin{itemize}
    \item \textbf{If the arbitrageur wins}, the payoff is \( v - g - b \).
    \item \textbf{If the arbitrageur loses}, the payoff is \( -(g \cdot r_1 + b \cdot r_2) \).
\end{itemize}

The probability of winning with bid \( b \) is given by the probability that all \( N-1 \) other arbitrageurs either abstain or bid less than \( b \). This probability is:
\[
\left( p + (1-p) F(b) \right)^{N-1}
\]
Thus, the expected payoff of bidding \( b \) is:
\[
\text{Payoff}(b) = \left( p + (1 - p) F(b) \right)^{N-1} (v - g - b) + \left( 1 - \left( p + (1 - p) F(b) \right)^{N-1} \right) (-g \cdot r_1 - b \cdot r_2)
\]


\subsection{Indifference Condition and Solving for \( p \)}

In a mixed strategy equilibrium, an arbitrageur must be indifferent between bidding and not bidding. That is, the expected payoff from bidding any \( b \) must be zero, the same as the expected payoff from abstaining. This leads to the following indifference condition:
\[
\left( p + (1 - p) F(b) \right)^{N-1} (v - g - b) = \left( 1 - \left( p + (1 - p) F(b) \right)^{N-1} \right) (g \cdot r_1 + b \cdot r_2)
\]
Let \( z = \left( p + (1-p) F(b) \right)^{N-1} \). Then, the indifference condition becomes:
\[
z (v - g - b) = (1 - z) (g \cdot r_1 + b \cdot r_2)
\]
Solving for \( z \):
\[
z = \frac{g \cdot r_1 + b \cdot r_2}{v - g - b + g \cdot r_1 + b \cdot r_2}
\]
Substitute \( z = \left( p + (1-p) F(b) \right)^{N-1} \) back into the equation:
\[
\left( p + (1 - p) F(b) \right)^{N-1} = \frac{g \cdot r_1 + b \cdot r_2}{v - g - b + g \cdot r_1 + b \cdot r_2}
\]
Taking the \((N-1)\)-th root on both sides:
\[
p + (1-p) F(b) = \left( \frac{g \cdot r_1 + b \cdot r_2}{v - g - b + g \cdot r_1 + b \cdot r_2} \right)^{\frac{1}{N-1}}
\]

\subsection{Solving for \( F(b) \)}

Isolating \( F(b) \):
\[
F(b) = \frac{1}{1 - p} \left( \left( \frac{g \cdot r_1 + b \cdot r_2}{v - g - b + g \cdot r_1 + b \cdot r_2} \right)^{\frac{1}{N-1}} - p \right)
\]

\subsection{Solving for \( p \) Using Boundary Condition}

We know that \( F(0) = 0 \). Substituting \( b = 0 \) into the expression for \( F(b) \):
\[
F(0) = \frac{1}{1 - p} \left( \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}} - p \right) = 0
\]
This simplifies to:
\[
p = \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}}
\]

\subsection{Verification at \( b = b^0 \)}

We verify that \( F(b^0) = 1 \), where \( b^0 = v - g \). Substituting \( b = b^0 \) into the expression for \( F(b) \):
\[
F(b^0) = \frac{1}{1 - p} \left( \left( \frac{vL \cdot r_1}{vL \cdot r_1} \right)^{\frac{1}{N-1}} - p \right) = 1
\]
Thus, the boundary condition \( F(b^0) = 1 \) holds, confirming the validity of the derived CDF.

==> archived-versions/Z-observations-comments.tex <==
\section{Observations And Comments}\label{app:observations}

\subsection{Impact of input parameters on probability to abstain, and bidding strategy}

\[
F(b) = \frac{1}{1 - p} \left( \left( \frac{g \cdot r_1 + b \cdot r_2}{v - g - b + g \cdot r_1 + b \cdot r_2} \right)^{\frac{1}{N-1}} - p \right)
\]

\[
p = \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}}
\]

\begin{itemize}
    \item $v$ (common value of the item being auctioned)
    \begin{enumerate}
    \item \textbf{Boundary conditions}:
    \begin{enumerate}
        \item $v$ needs to be greater than the minimum cost of winning ($g$), for anyone to bid.
        \item At $v = g$, $ p = 1 $, which is consistent with the intuition that if winning does not generate any positive profit, then no one will bid.
    \end{enumerate}

        \item \textbf{Impact on participation}:\\
        $p$ is decreasing in $v$, meaning as the item being auction gets more and more valuable, the probability to abstain from the auction becomes lower and lower.
    \end{enumerate}

    \item $N$ (number of participants)
    \begin{enumerate}
        \item  \textbf{Impact on participation}:  \\ Since the fraction is less than 1, raising it to the $N-1$ power makes it closer to 1. This means as the number of participants increases, the probability that each one will choose to bid in any round decreases. This makes sense, because as the number of bidders increase, the probability for anyone to win in a given auction decreases, so it makes sense to abstain more everything else equal.
        \item \textbf{Impact on bidding strategy}: \\
        As $N$ increases, $F(b)$ grows faster when $b$ is small and slower when $b$ is large, which indicates that when number of participants increases, conditional on bidding, they choose to bid less aggressively in order to capture more potential profit if they win.
    \end{enumerate}

    \item $g$ (minimum bid)
    \begin{enumerate}
        \item $p$ is increasing in $g$, so increasing minimum bid will decrease participation rate
    \end{enumerate}

    \item $r_1$ (fraction of minimum bid that is paid in case of loss)

        \[ \frac{dp}{dr_1} = \frac{1}{N-1} \cdot p^{2-N} \cdot \frac{g \cdot (v-g)}{(v - g + g \cdot r_1)^2} \]
        Since this is always positive, increasing the fraction of minimum bid that needs to be paid in case of loss will increase the probability of each bidder abstaining.

    \item $r_2$ (fraction of additional bid that is paid in case loss)

        Note that $r_2$ is not part of $p$, and therefore does not play a role in the decision to bid. However, it is a part of $F(b)$, and therefore plays a role in the bidding strategy conditional on bidding.
\end{itemize}

\iffalse
\subsection{Proof strategy for expected bid comparative statics}

If $\partial F/\partial\theta\geq0$ where $\theta$ is some parameter of interest, then the CDF increases pointwise for all $b\in[0,V-g]$. Then for any $\theta_1,\theta_2$ such that $\theta_1<\theta_2$, letting $X_{\theta_1}\sim F_{\theta_1}$ and $X_{\theta_2}\sim F_{\theta_2}$, it follows that $X_{\theta_1}$ stochastically dominates $X_{\theta_2}$ in the first order, so $\mathbb{E}X_{\theta_1}>\mathbb{E}X_{\theta_2}$. Vice-versa if $\d=\partial F/\partial\theta\leq0$.

Given our equilibrium bidding CDF, we have
\begin{gather*}
    \frac{\partial F}{\partial N} = -\frac{\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right)^{\frac{1}{N-1}}}{(1-p)(N-1)^2}\log\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right) \geq 0 \\[0.25\baselineskip]
    \frac{\partial F}{\partial V} = -\frac{\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right)^{\frac{1}{N-1}}}{(1-p)(N-1)(V-g-b+r_1g+r_2b)}\leq0 \\[0.25\baselineskip]
    \frac{\partial F}{\partial r_1} = \frac{g(V-g-b)\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right)^{\frac{1}{N-1}}}{(1-p)(N-1)(r_1g+r_2b)(V-g-b+r_1g+r_2b)}\geq0 \\[0.25\baselineskip]
    \frac{\partial F}{\partial r_2} = \frac{b(V-g-b)\left(\frac{r_1g+r_2b}{V-g-b+r_1g+r_2b}\right)^{\frac{1}{N-1}}}{(1-p)(N-1)(r_1g+r_2b)(V-g-b+r_1g+r_2b)}\geq0
\end{gather*}


\subsection{Impact of different input parameters on model equilibrium results}

In the final outcome, we care about a few different outcomes.

\begin{enumerate}
    \item Percentage of times an auction has participation \\
    This is important because when an arbitrage opportunity left untouched, overall welfare (defined below) decreases, and overall market efficiency lowers.
    The expression is $1 - p^N$, which can be expanded to be
    \[
    1 - p^N = 1 - \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{N}{N-1}}
    \]
    Denote this value $P$.

    \begin{enumerate}
        \item $N$ \\
        \[
        \frac{dP}{dN} =  \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{N}{N-1}} \cdot \ln \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right) \cdot \frac{1}{(N-1)^2} < 0
        \]
        $P$ is decreasing in $N$, and we observe that
        \[
        \lim_{N \to \infty} P = 1 - \frac{g \cdot r_1}{v - g + g \cdot r_1}.
        \]


        \item $v$ \\
        \[
        \frac{dP}{dv} = \frac{N}{N-1} \cdot \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{N}{N-1} - 1} \cdot \left( \frac{g \cdot r_1}{(v - g + g \cdot r_1)^2} \right) > 0
        \]

        $P$ is increasing in $v$, and as $v \to \infty$, $P \to 1$


        \item $g$ \\
        It's obvious to see that $P$ decreases in $g$, which makes sense because a higher minimum bid discourages participation.

        \item $r_1, r_2$ \\
        $P$ decreases in $r_1$, and does not change with respect to $r_2$.

    \end{enumerate}

    \item Total welfare \\

    This is sum of all payments collected.
    First we note that when $v < g$, no big will be submitted, and total welfare will be 0.

    Note that since all bidders are in a competitive environment, the expected profit is 0. This means the expected amount of total payment is equal to the total value of items sold. In our auction setting, as long as at least one participant choose to bid, the item will be sold. The probability that all participants choose to abstain is $1 - P$, so the item will be sold with probability $P$. The expected value of item sold is therefore $v \times P$

    Given the above, this value can be written as

    \[
    v \times P = v \times \left(1 - \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{N}{N-1}} \right)
    \]

    Since the total realizable amount of welfare is simply $v$, the amount of loss is then
    \[
    v \times (1-P) = v \times \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{N}{N-1}}
    \]

    Denote this as $W_L$.

    \begin{enumerate}
        \item $N$ \\
        Since $v$ is independent from $N$, the direction of effect from $N$ on $W_L$ is the same as the effect of $N$ on $-P$.  We know that $P$ is decreasing in $N$, so $W_L$ increases in $N$. Furthermore, from the previously computed limit, we know that
        \[
        \lim_{N \to \infty} W_L = v \times  \frac{g \cdot r_1}{v - g + g \cdot r_1}
        \]

        \item $g$ \\
        $W_L$ is increasing in $g$. When $g=0$, $W_L=0$

        \item $r_1$ \\
        $W_L$ increases in $r_1$ when $v>g$; however, when $v<g$, reducing $r_1$ has no effect on welfare.

        \item $r_2$ \\
        $W_L$ does not change with $r_2$.
    \end{enumerate}

    \item Number of submitted bids (esp. as $N \to \infty$) \\
    This is simply $N \times (1-p)$. Since $p$ is a function of $N$, we can further expand as
    \[
    N \times (1 - p) = N \times \left( 1 - \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}} \right)
    \]

    Taking the limit as \( N \to \infty \):

    \[
    \lim_{N \to \infty} N \times (1 - p) = \lim_{N \to \infty} N \times \left( 1 - \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}} \right)
    \]

    Using the approximation for small exponents:

    \[
    1 - \left( \frac{g \cdot r_1}{v - g + g \cdot r_1} \right)^{\frac{1}{N-1}} \approx \frac{1}{N-1} \cdot \ln\left( \frac{v - g + g \cdot r_1}{g \cdot r_1} \right)
    \]

    Thus, multiplying by \( N \) and taking the limit:

    \[
    \lim_{N \to \infty} N \times (1 - p) = \ln\left( \frac{v - g + g \cdot r_1}{g \cdot r_1} \right)
    \]

    Note that the number of bids remains finite when $g >0, $, and roughly scales with the log of $v$, when $v \gg g$.



    \item Sequencer revenue, in the presence of MEV tax \\
    We first note that total welfare does not change with $r_2$. This means that when $r_2 \neq r_1$, the only thing that changes is the composition of total revenue (from minimum bid vs. additional bid collected), but not the total payment collected. In the context of sequencer revenue with presence of MEV tax, we can derive the expression for MEV tax revenue vs. sequencer revenue. See  \ref{sec:mev_tax}
\end{enumerate}
\fi

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> old/old1-intro.tex <==
\section{Introduction}
\subsection{Introducing the problem}

In this analysis, we explore the strategic behavior of arbitrageurs in a blockchain environment where they compete to exploit price discrepancies between a decentralized exchange (DEX) and a centralized exchange (CEX). The blockchain uses a Priority Gas Auction (PGA) for ordering transactions, and we focus on the scenario with Non-Revert Protection (NRP), where losing arbitrageurs still incur a cost proportional to their bid.



==> old/old10-conclusion.tex <==
\section{Conclusion and Future Work}
We summarize our findings, highlighting the impact of revert protection on arbitrageur behavior and its implications for sequencer revenue, LP profitability, and price discovery. Potential avenues for future research include the impact of dynamic gas pricing and the integration of Layer 1 dynamics into the model.

==> old/old2-related-work.tex <==
\section{Related Work}
\subsection{arbitrage behavior on eth mainnet}
\subsection{arbitrage modeling in tradfi }
\subsection{lp profitability}
\subsection{onchain price discovery}
\subsection{sequencing rule choices, if any??}

We review prior research on arbitrage in traditional finance and blockchain ecosystems, focusing on arbitrage in decentralized exchanges (DEXs) and the role of PGA-ordered systems in Layer 2 rollups. Our work extends existing literature by modeling arbitrage dynamics with and without revert protection.


==> old/old3-motivation.tex <==
\section{Motivation}
\subsection{Why Layer 2 and Sequencers?}
Layer 2 scalability solutions, like optimistic rollups, are essential for scaling Ethereum. Sequencers in Layer 2 manage transactions and prioritize them through gas auctions, making their behavior crucial to understand.

\subsection{Why PGA and Arbitrage?}
Priority Gas Auction (PGA) systems are vital for ordering transactions in L2 chains. Arbitrageurs help stabilize prices between DEXs and CEXs, and their behavior directly impacts the efficiency of price discovery.

\subsection{Implications for LPs and DeFi}
Arbitrage affects LP profitability, as inefficient arbitrage dynamics can lead to adverse selection. Revert protection may mitigate these effects, making it critical to model.


==> old/old4-model-setup.tex <==
\section{Model Setup}
\subsection{Blockchain Environment}
\begin{enumerate}
    \item The blockchain is an optimistic roll-up of Ethereum with a single sequencer.
    \item The sequencer generates revenue from base fees and priority fees.
    \item Sequencer costs are not explicitly modeled but incurred during data posting to Ethereum.
\end{enumerate}

\subsection{Market Structure}
\begin{enumerate}
    \item A DEX pool trades two assets.
    \item These assets are also traded on a centralized exchange (CEX), creating CEX-DEX arbitrage opportunities.
    \item The L2 chain has a block time \( b \), during which price discrepancies may emerge.
\end{enumerate}

\subsection{Arbitrageurs and Transaction Ordering}
\begin{enumerate}
    \item N arbitrageurs compete in a PGA-ordered chain, with priority determined by the gas bid.
    \item They exploit discrepancies between CEX price \( p_c \) and DEX price \( p_d \).
\end{enumerate}

\subsection{Gas Fee Structure}
\begin{enumerate}
    \item \textbf{Success Gas Cost:} \( g + b \) (base fee plus priority fee).
    \item \textbf{Revert Gas Cost:} \( (g + b) \times r \), where \( r \) is the revert penalty fraction.
\end{enumerate}




\section*{Model Setup}

\subsection*{Blockchain Environment}
\begin{enumerate}
    \item The blockchain is an optimistic roll-up of Ethereum with a single sequencer.
    \item The sequencer generates revenue from base fees and priority fees.
    \item The sequencer incurs costs when posting data to Ethereum, primarily from data posting (but we are not going to model this part).
\end{enumerate}

\subsection*{Market Structure}
\begin{enumerate}
    \item There is one DEX pool trading two assets.
    \item These assets are also continuously traded on a centralized exchange (CEX), creating opportunities for CEX-DEX arbitrage.
    \item The L2 chain has a block time of $b$ seconds, during which the price on the DEX may remain stale compared to the CEX, creating arbitrage opportunities.
\end{enumerate}

\subsection*{Transaction Ordering and Arbitrageurs}
\begin{enumerate}
    \item The chain has a private mempool and orders transactions by priority fees within each block.
    \item There are $N$ equally skilled arbitrageurs.
    \item They compete for arbitrage opportunities when there is a price discrepancy between the CEX price ($p_c$) and the DEX price ($p_d$).
\end{enumerate}

\subsection*{Fee Rate and Trading Dynamics}
\begin{itemize}
    \item \textbf{Trading Fee Rate $f$}: The fee rate for trading in the AMM pool.
    \item \textbf{Price Discrepancy Threshold}: Arbitrage is possible when the price difference exceeds the fee rate. However, successful arbitrage also depends on having a positive expected value after accounting for costs.
\end{itemize}

\subsection*{Gas Fee Structure}
To simplify the math, let's assume there's a fixed gas fee, and a variable priority fee (or "bid"). If a transaction reverts, the sender will have to pay a fixed fraction of their bid.

\begin{enumerate}

    \item \textbf{Gas Used for Success}: $g + b$.
    \item \textbf{Gas Used for Revert }: $(g + b) * r$
\end{enumerate}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> old/old5-arbitrage-analysis.tex <==
\section{Arbitrage Analysis (Economics of a Single Successful Arbitrage)}

\todo{I don't think the details of the arbitrage are important. Can we just say that the
  opportunity has a value $V$, which is common to all participants. This theory could apply to an
  AMM or simpler situations like an auction.}

\subsection{Volume Calculation}

- \textbf{Liquidity Depth $L$}: Represents the liquidity depth per unit price change.
- \textbf{Volume Formula}: The volume of an arbitrage transaction on the DEX depends on the price difference and liquidity depth:
  \[
  \text{Volume} = (p_d - p_{\text{dex-stop}}) \times L
  \]
  where $p_{\text{dex-stop}}$ is the price at which arbitrage is no longer profitable (see below).

\subsection{Case 1: \( p_d \times (1-f) > p_c \) (DEX Price Too High)}

\begin{enumerate}
  \item \textbf{Sell on DEX}:
    \begin{itemize}
      \item \textbf{Traded Volume}: \( (p_d - \frac{p_c}{1 - f}) \times L \)
      \item \textbf{Average Price}: \( \frac{p_d + \frac{p_c}{1 - f}}{2} \)
      \item \textbf{Proceeds from Selling on DEX}:
        \[
        \text{Revenue} = \left(\frac{p_d + \frac{p_c}{1 - f}}{2}\right) \times \left(p_d - \frac{p_c}{1 - f}\right) \times L
        \]
    \end{itemize}

  \item \textbf{Buy on CEX}:
    \begin{itemize}
      \item Buys the same volume on CEX, at \( p_c \)
      \item \textbf{Cost on CEX}: \( p_c \times \left(p_d - \frac{p_c}{1 - f}\right) \times L \)
    \end{itemize}

  \item \textbf{Trading Fee}:
    \begin{itemize}
      \item \textbf{Trading Fee}: \( f \times \left(p_d - \frac{p_c}{1 - f}\right) \times L \)
    \end{itemize}

  \item \textbf{Fixed Costs}:
    \begin{itemize}
      \item \textbf{Gas Fee}: \( g + b \)
    \end{itemize}

  \item \textbf{Net Profit}:
    \[
    \text{Net Profit} = \text{Revenue} - \text{Cost} - \text{Trading Fee} - \text{Gas Fee}
    \]
    \[
    \text{Net Profit} = \left(\frac{\left(p_d - \frac{p_c}{1 - f}\right)^2}{2}\right) \times L - (g + b)
    \]
\end{enumerate}

\subsection{Case 2: \( p_d \times (1+f) < p_c \) (DEX Price Too Low)}

\begin{enumerate}
  \item \textbf{Buy on DEX}:
    \begin{itemize}
      \item \textbf{Traded Volume}: \( \left(\frac{p_c}{1 + f} - p_d\right) \times L \)
      \item \textbf{Average Price}: \( \frac{p_d + \frac{p_c}{1 + f}}{2} \)
      \item \textbf{Cost on DEX}:
        \[
        \text{Cost} = \left(\frac{p_d + \frac{p_c}{1 + f}}{2}\right) \times \left(\frac{p_c}{1 + f} - p_d\right) \times L
        \]
    \end{itemize}

  \item \textbf{Sell on CEX}:
    \begin{itemize}
      \item \textbf{Revenue on CEX}: \( p_c \times \left(\frac{p_c}{1 + f} - p_d\right) \times L \)
    \end{itemize}

  \item \textbf{Trading Fee}:
    \begin{itemize}
      \item \textbf{Trading Fee}: \( f \times \left(\frac{p_c}{1 + f} - p_d\right) \times L \)
    \end{itemize}

  \item \textbf{Fixed Costs}:
    \begin{itemize}
      \item \textbf{Gas Fee}: \( g + b \)
    \end{itemize}

  \item \textbf{Net Profit}:
    \[
    \text{Net Profit} = \text{Revenue} - \text{Cost} - \text{Trading Fee} - \text{Gas Fee}
    \]
    \[
    \text{Net Profit} = \left(\frac{\left(\frac{p_c}{1 + f} - p_d\right)^2}{2}\right) \times L - (g + b)
    \]
\end{enumerate}

\subsection{Common Expression for Net Profit for a Successful Arb}

The net profit can be expressed using a common formula for both cases:

\[
\text{Net Profit} = v \times L - (g + b)
\]
where
\[
v = \frac{(p_d - \frac{p_c}{1 \pm f})^2}{2}
\]
and either \( p_d - \frac{p_c}{1 - f} \geq 0 \) or  \( \frac{p_c}{1 + f} - p_d \geq 0 \).

Note that the break-even bid is 
\[
b^0 = v \times L - g
\]

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> old/old6-nash-equilibrium-analysis.tex <==


\section{Nash Equilibrium Analysis}
\subsection{Fixed Strategy Analysis}
We analyze whether arbitrageurs could adopt a fixed strategy by bidding the same amount \( b^* \). A fixed strategy equilibrium cannot exist, as each arbitrageur has an incentive to slightly increase their bid to ensure winning.

\subsection{Mixed Strategy Nash Equilibrium}
In the mixed strategy Nash equilibrium, arbitrageurs randomize over a range of possible bids. The CDF \( F(b) \) describes the distribution of bids, with a fraction \( 1-p \) of arbitrageurs bidding and \( p \) abstaining.



\section*{Fixed Strategy Analysis}

Given the new gas cost structure, let's revisit the possibility of a fixed strategy Nash Equilibrium, where all arbitrageurs choose the same bid \( b^* \).

A fixed strategy \( b^* \) cannot exist because:
    \begin{itemize}
        \item No one is incentivized to bid over profit in a success (therefore $ b^* \leq b^0$).
        \item Since a revert has a positive cost, if all bidders bid net profit conditional on success, then overall the expected value must be negative. Therefore, everyone bidding net profit conditional on success is not an equilibrium. (therefore $ b^* < b^) $
        \item If all arbitrageurs bid \( b^* \), which is less than net profit in a success, then there is always an incentive to slightly increase the bid. 
        \item A slight increase in the bid ensures winning, which will result in a positive net profit with probability 1. (therefore any $b < b^0$ cannot be $b^*$)
        \item This constant incentive to deviate from \( b^* \) means a fixed strategy is unstable.

    \end{itemize}

    \todo{This is proving there is no symmetric pure strategy equilbrium, would be strong to show
      there is no pure strategy equilibrium full stop. Also I don't think ``fixed strategy'' is a
      game theory term, people sare pure strategy or deterministic strategy.}


\section*{Mixed Strategy Nash Equilibrium}

Given the instability of a fixed strategy, we analyze a mixed strategy Nash Equilibrium, where arbitrageurs randomize their bids within a certain range.

\subsection*{Mixed Strategy and CDF Derivation}

In a mixed strategy equilibrium, each arbitrageur randomizes over a range of possible bids. Let \( p \) denote the probability that an arbitrageur chooses not to bid at all. For those who decide to bid, their bids are distributed according to a cumulative distribution function (CDF) \( F(b) \), which determines the probability of bidding strictly less than a given bid \( b \).


\subsection*{Expected Payoff from Bidding}

Say there are N arbitrageurs. Let \( b \) denote the priority fee (tip) that an arbitrageur chooses to bid. The total expected payoff for an arbitrageur who bids \( b \) is given by:

\[
\text{Expected Payoff}(b) = (1-p) \times \left[\sum_{i=0}^{N-1} P(\text{win} \mid i) \times \text{Payoff}(\text{win} \mid i) + \sum_{i=0}^{N-1} P(\text{lose} \mid i) \times \text{Payoff}(\text{lose} \mid i)\right]
\]

Here:
\begin{itemize}
    \item \( (1-p) \) is the probability that the arbitrageur decides to bid.
    \item \( P(\text{win} \mid i) \) is the probability that the arbitrageur's bid \( b \) wins (i.e., is the highest bid) given that \( i \) other arbitrageurs also bid, and the rest passes on the opportunity.
    \item \( P(\text{lose} \mid i) = 1 - P(\text{win} \mid i) \) is the probability that the arbitrageur's bid loses, given that \( i \) other arbitrageurs bid.
    \item \( \text{Payoff}(\text{win} \mid i) \) is the conditional payoff if the arbitrageur wins the bid.
    \item \( \text{Payoff}(\text{lose} \mid i) \) is the conditional payoff if the arbitrageur loses the bid, which typically includes the cost of the revert penalty.
\end{itemize}

\subsection*{Conditional Payoffs}

\paragraph{Winning Payoff:}
The payoff from winning the bid, given \( i \) other bidders, is:

\[
\text{Payoff}(\text{win} \mid i) = v \times L - b - g
\]

This expression accounts for:
\begin{itemize}
    \item \( v \times L \): The value of the arbitrage opportunity.
    \item \( b \): The priority fee (tip) paid to secure the transaction.
    \item \( g \): The gas fee required to execute the transaction successfully.
\end{itemize}

\paragraph{Losing Payoff:}
The payoff from losing the bid, given \( i \) other bidders, is:

\[
\text{Payoff}(\text{lose} \mid i) = -(g + b) \times r
\]

This expression reflects the costs incurred when the transaction reverts (fails), including:
\begin{itemize}
    \item \( g \times r \): The gas cost reduced by the revert penalty factor.
    \item \( b \times r \): The priority fee, which is also scaled by the revert penalty factor.
\end{itemize}

\subsection*{Probability of Winning or Losing}

The probability that an arbitrageur’s bid \( b \) wins given \( i \) other bidders is represented by the cumulative distribution function \( F(b) \), which describes the distribution of bids among all arbitrageurs. Specifically:

\[
P(\text{win} \mid i) = F(b)^i
\]

This probability is the likelihood that all \( i \) other arbitrageurs have bids less than \( b \), ensuring that the arbitrageur wins.

The probability of losing, given that \( i \) other bidders also participate, is:

\[
P(\text{lose} \mid i) = 1 - F(b)^i
\]

\subsection*{Overall Expected Payoff}

Combining these elements, the overall expected payoff for an arbitrageur who bids \( b \) is:


\[
\text{Expected Payoff}(b) = (1-p) \times \left[ \sum_{i=0}^{N-1} \binom{N-1}{i} (1-p)^i p^{N-1-i} \left( F(b)^i \times (v \times L - b - g) \right. \right.
\]
\[
\left. \left. - (1-F(b)^i) \times (g + b) \times r \right) \right]
\]

This expression reflects the weighted sum of the conditional payoffs across all possible numbers of other bidders \( i \), weighted by the binomial probability distribution of \( i \), which depends on the mixed strategy probability \( p \).


Expanding the binomial expression:



\[
\text{Expected Payoff}(b) = (1-p) \times \left[\left(p + (1-p)F(b)\right)^{N-1} \times 
(v \times L - b \times (1 - r) - g \times (1 - r)) - (g + b) \times r\right]
\]




\section*{Deriving the CDF \( F(b) \)}

In a mixed strategy equilibrium, arbitrageurs must be indifferent between bidding any amount \( b \) and not bidding at all. The expected payoff from bidding \( b \) must therefore equal the expected payoff from not bidding, which is zero.

\subsection*{Expected Payoff Function}

The expected payoff for an arbitrageur who bids \( b \) is given by:

\[
\text{Expected Payoff}(b) = (1-p) \times \left[\left(p + (1-p)F(b)\right)^{N-1} \times 
(v \times L - b \times (1 - r) - g \times (1 - r)) - (g + b) \times r\right]
\]

Since the arbitrageur must be indifferent between bidding and not bidding, we set the expected payoff equal to zero:

\[
(1-p) \times \left[\left(p + (1-p)F(b)\right)^{N-1} \times 
(v \times L - b \times (1 - r) - g \times (1 - r)) - (g + b) \times r\right] = 0
\]

\subsection*{Simplifying the Indifference Condition}

For the expected payoff to be zero, the term inside the brackets must equal zero:

\[
\left[\left(p + (1-p)F(b)\right)^{N-1} \times 
(v \times L - b \times (1 - r) - g \times (1 - r))\right] = (g + b) \times r
\]

We then solve for \( F(b) \):

\[
\left(p + (1-p)F(b)\right)^{N-1} = \frac{(g + b) \times r}{v \times L - b \times (1 - r) - g \times (1 - r)}
\]

Taking the \((N-1)\)th root on both sides:

\[
p + (1-p)F(b) = \left[\frac{(g + b) \times r}{v \times L - b \times (1 - r) - g \times (1 - r)}\right]^{\frac{1}{N-1}}
\]

Finally, solve for \( F(b) \):

\[
F(b) = \frac{1}{1-p} \left[\left[\frac{(g + b) \times r}{v \times L - b \times (1 - r) - g \times (1 - r)}\right]^{\frac{1}{N-1}} - p\right]
\]

\subsection*{Boundary Conditions}

The derived CDF \( F(b) \) must satisfy the following boundary conditions:

\begin{itemize}
    \item \textbf{At \( b = 0 \)}: \( F(0) = 0 \). \\
    Setting \( b = 0 \) should lead to the lowest probability of winning, so the CDF should start at zero.
    
    \item \textbf{At \( b = vL - g \)}: \( F(vL - g) = 1 \). \\
    Setting \( b = vL - g \) should make the CDF equal to 1, representing the maximum possible bid.
\end{itemize}

This ensures that the CDF \( F(b) \) behaves as expected in the context of the arbitrage model and fulfills the indifference condition required for a mixed strategy equilibrium.





\section*{Solving for \( p \) and Verifying Boundary Conditions}

\subsection*{Solving for \( p \) using \( F(0) = 0 \)}

We previously derived the cumulative distribution function \( F(b) \):

\[
F(b) = \frac{1}{1-p} \left[\left[\frac{(g + b) \times r}{v \times L - b \times (1 - r) - g \times (1 - r)}\right]^{\frac{1}{N-1}} - p\right]
\]

Setting \( b = 0 \) to satisfy the boundary condition \( F(0) = 0 \):

\[
F(0) = \frac{1}{1-p} \left[\left[\frac{g \times r}{v \times L - g \times (1 - r)}\right]^{\frac{1}{N-1}} - p\right] = 0
\]

This simplifies to:

\[
p = \left[\frac{g \times r}{v \times L - g \times (1 - r)}\right]^{\frac{1}{N-1}}
\]

\subsection*{Verifying \( F(vL - g) = 1 \)}

Next, we verify the boundary condition \( F(vL - g) = 1 \) using the derived \( p \):

\[
F(vL - g) = \frac{1}{1-p} \left[\left[\frac{vL \times r}{vL \times r}\right]^{\frac{1}{N-1}} - p\right] = \frac{1}{1-p} \left[1 - p\right] = 1
\]

The boundary condition \( F(vL - g) = 1 \) holds true, confirming that the derived value of \( p \) is consistent with the mixed strategy Nash equilibrium.

\section*{Summary}

In the context of a competitive blockchain environment with Non-Revert Protection (NRP), arbitrageurs randomize their bids according to a mixed strategy characterized by a cumulative distribution function (CDF) \( F(b) \) and a probability \( p \) of not bidding at all.

\subsection*{CDF \( F(b) \)}

The functional form of the CDF \( F(b) \) is derived as:

\[
F(b) = \frac{1}{1-p} \left[\left[\frac{(g + b) \times r}{v \times L - b \times (1 - r) - g \times (1 - r)}\right]^{\frac{1}{N-1}} - p\right]
\]

where:
\begin{itemize}
    \item \( g \) is the base gas fee.
    \item \( r \) is the revert penalty factor.
    \item \( vL \) is the value of the arbitrage opportunity, where \( v = \frac{(|p_d - p_c| - f)^2}{2} \).
    \item \( N \) is the number of arbitrageurs.
    \item \( p \) is the probability of not bidding, derived as:
\end{itemize}

\[
p = \left[\frac{g \times r}{v \times L - g \times (1 - r)}\right]^{\frac{1}{N-1}}
\]

This mixed strategy equilibrium ensures that arbitrageurs are indifferent between bidding any amount \( b \) and not bidding at all, as their expected payoff in both cases is zero.


\subsection{Revert Protection as a Special Case}
We show that Revert Protection (RP) is a special case of Non-Revert Protection (NRP) by setting \( r = 0 \). This reduces the revert gas cost to zero, and the mixed strategy equilibrium derived for NRP applies directly to RP. In this section, we compare the mixed strategy behaviors of arbitrageurs under both regimes, analyzing how the absence of revert costs in RP affects gas bids, sequencer revenue, and LP profitability.

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> old/old7-impact-on-onchain-economics.tex <==

\section{Price Discovery, LP Profitability, and Sequencer Revenue}

\subsection{Price Discovery and Deviation}
Price deviations between CEX and DEX are corrected by arbitrage. We discuss how revert costs in NRP reduce the frequency of arbitrage, leading to larger price deviations compared to RP, where arbitrage occurs more frequently.


\subsection{LP Profitability and Adverse Selection Loss}
LPs lose \( vL \) when arbitrage occurs, but collect fees on each transaction. We compare how RP and NRP affect LP profitability, focusing on the adverse selection problem caused by arbitrage opportunities.


\subsection{Sequencer Revenue}
We calculate sequencer revenue by summing the gas fees collected from winning bids and reverted transactions. In RP, only winning bids contribute to sequencer revenue, while in NRP, reverted transactions also provide revenue.

\[
\begin{split}
\text{sequencer revenue} & = Np \times E\left[ \left\{ r + \left( 1 - p + p F(b)\right)^{N-1}  (1-r)\right\}(g + b) \right] \\
\end{split}
\]

\[
\begin{split}
\text{welfare} & =  V (1-p^N)
\end{split}
\]

\[
\begin{split}
\text{sequencer revenue} & =  V \left(1-p^N\right) \\
& = V\left( 1 - \left( \frac{gr}{V-g(1-r)} \right)^{\frac{N}{N-1}} \right) \\
& \xrightarrow[N\rightarrow\infty]{}
V\left( 1 - \frac{gr}{V-g(1-r)}  \right)
\end{split}
\]


==> old/old8-simulation.tex <==
\section{Numerical Simulations}
We simulate arbitrage dynamics under different parameter values (gas fees, liquidity depth, volatility) to validate our theoretical results. The simulations compare sequencer revenue, LP profitability, and price discovery under RP and NRP.


\subsection{Data Generation Process for On-Chain Arbitrage Simulation}

\subsubsection{Generating the "True Price" Series}

\begin{enumerate}
    \item The "true price" at time $t$, denoted as $p_{\text{true}}(t)$, follows a Brownian motion process with drift $\mu$ and volatility $\sigma$:
    \[
    dp_{\text{true}}(t) = \mu p_{\text{true}}(t) dt + \sigma p_{\text{true}}(t) dW(t)
    \]
    where $dW(t)$ represents the increment of a Wiener process (standard Brownian motion).

    \item The simulation runs from time $t = 0$ to $t = T$, with time discretized into blocks. Each block has a duration of $\text{block\_time}$, which is a parameter in the simulation.
\end{enumerate}

\subsubsection{Generating the "On-Chain Price" Series}

\begin{enumerate}
    \item[2.1] \textbf{Initial Condition}: At time $t = 0$, the on-chain price is set to be equal to the true price:
    \[
    p_{\text{onchain}}(0) = p_{\text{true}}(0)
    \]

    \item[2.2] \textbf{Sequential Price Updates}: For each time increment from $t = 0$ to $t = T$, the on-chain price $p_{\text{onchain}}(t)$ is updated based on the price difference between $p_{\text{onchain}}(t-1)$ and $p_{\text{true}}(t)$. The process is as follows:

    \begin{enumerate}
        \item[2.2.1] \textbf{Increment Time}: Increment time by one block, where the block duration is given by $\text{block\_time}$. At each increment, the true price $p_{\text{true}}(t)$ evolves according to the Brownian motion process.
        
        \item[2.2.2] \textbf{On-Chain Price Stays Stale}: The on-chain price remains unchanged unless an arbitrage event occurs. The true price continues to evolve according to the Brownian motion dynamics, while the on-chain price remains the same until arbitrage forces a correction.

        \item[2.2.3] \textbf{Arbitrage Opportunity Detection}: At each time increment, calculate the price difference between the current true price and the previous on-chain price:
        \[
        \Delta p(t) = |p_{\text{true}}(t) - p_{\text{onchain}}(t-1)|
        \]
        An arbitrage opportunity exists if:
        \[
        \Delta p(t) > f
        \]
        where $f$ is the pool fee rate. 
        
        \begin{itemize}
            \item If no arbitrage opportunity is detected, increment the time by $\text{block\_time}$ and repeat the process.
            \item If an arbitrage opportunity exists, compute the probability $p$ that an arbitrageur passes on the opportunity. The probability that no arbitrageur takes action is $p^N$, where $N$ is the number of arbitrageurs.
            
            \item Perform a binary draw with probabilities $(p^N, 1 - p^N)$ to determine if any arbitrage occurs. 
            \begin{itemize}
                \item If no arbitrage occurs, increment the time by $\text{block\_time}$ and repeat the process.
                \item If arbitrage occurs, the on-chain price is updated as described below.
            \end{itemize}
        \end{itemize}

        \item[2.2.4] \textbf{Arbitrage Update}: When an arbitrage occurs, the on-chain price is updated to the boundary determined by the true price and the pool fee rate:
        \[
        p_{\text{onchain}}(t) = 
        \begin{cases}
        p_{\text{true}}(t) + f & \text{if } p_{\text{onchain}}(t-1) > p_{\text{true}}(t) + f \\
        p_{\text{true}}(t) - f & \text{if } p_{\text{onchain}}(t-1) < p_{\text{true}}(t) - f
        \end{cases}
        \]
    \end{enumerate}

    \item[2.3] \textbf{Repeat Until Time $T$}: The process repeats from steps 2.2.1 to 2.2.4 until the simulation reaches the final time $t = T$.
\end{enumerate}


\section*{Onchain Price Discovery Statistics}

\textbf{Motivation:}  
The ability of the onchain price to track the true price accurately is crucial for maintaining market integrity and ensuring that decentralized exchanges (DEXs) offer fair prices to participants. In our model, onchain prices can deviate from true prices due to arbitrageur behavior, pool fees, and transaction costs. Measuring the quality of price discovery helps evaluate how efficiently the arbitrage mechanism works and whether revert protection (or the lack thereof) affects price accuracy. Price discovery quality is expected to be highest when the onchain price remains close to the true price, within the arbitrage-free band set by the pool fee rate.

\textbf{Steps to Compute:}  
To evaluate price discovery quality, we will implement the following metrics during simulation:

\begin{itemize}
    \item \textbf{Mean Absolute Deviation (MAD)}: This will measure the average absolute deviation between the onchain price and the true price over the course of the simulation. At each time step $t$, we compute:
    \[
    \text{MAD} = \frac{1}{T} \sum_{t=0}^{T} \left| p_{\text{onchain}}(t) - p_{\text{true}}(t) \right|
    \]
    This will be implemented by iterating over the time steps and recording the deviation between the onchain and true prices.

    \item \textbf{Deviation Beyond Fee Band (DBF)}: This metric will track how frequently the onchain price deviates by more than the pool fee rate ($f$) from the true price:
    \[
    \text{DBF} = \frac{1}{T} \sum_{t=0}^{T} \mathbb{1} \left( |p_{\text{onchain}}(t) - p_{\text{true}}(t)| > f \right)
    \]
    We will record the number of times the onchain price exceeds this deviation threshold and calculate its frequency over time.
    
    \item \textbf{Max Deviation (MD)}: This metric will record the maximum observed deviation between the onchain price and the true price during the entire simulation:
    \[
    \text{MD} = \max_{t} \left( |p_{\text{onchain}}(t) - p_{\text{true}}(t)| \right)
    \]
    This statistic will help capture extreme events where the onchain price fails to follow the true price for an extended period.
\end{itemize}

\section*{LP Profitability Statistics}

\textbf{Motivation:}  
Liquidity providers (LPs) in an AMM face a trade-off between earning fees from arbitrage transactions and losing money due to price divergence between the true price and the onchain price. LP profitability is therefore driven by two opposing forces: (1) the fees they collect when arbitrageurs trade, and (2) their exposure to adverse selection losses when prices move against them. By understanding LP profitability, we can evaluate the impact of arbitrage frequency and price deviations on LPs' financial performance.

\textbf{Steps to Compute:}  
We propose the following metrics to quantify LP profitability dynamics:

\begin{itemize}
    \item \textbf{Cumulative Fees Earned (CFE)}: This will track the total amount of fees earned by LPs due to arbitrage transactions during the simulation. For each arbitrage transaction at time $t$, the fees earned are given by:
    \[
    \text{CFE}(T) = \sum_{t=0}^{T} f \times \text{Volume}(t)
    \]
    where $f$ is the LP fee rate and $\text{Volume}(t)$ is the traded volume at time $t$.

    \item \textbf{Cumulative Adverse Selection Loss (CASL)}: This will track the total amount of money lost by LPs due to arbitrageurs exploiting price discrepancies. The adverse selection loss is proportional to the deviation between the true price and the average price at which LPs are trading. It is given by:
    \[
    \text{CASL}(T) = \sum_{t=0}^{T} \left( \frac{|p_{\text{true}}(t) - p_{\text{onchain}}(t)|}{2} \times \text{Volume}(t) \right)
    \]
    This measures how much LPs lose when arbitrageurs take advantage of stale onchain prices.

    \item \textbf{Net LP Profitability (NLP)}: LPs’ overall profitability is determined by their fee income minus their losses due to adverse selection. Thus, we calculate:
    \[
    \text{NLP}(T) = \text{CFE}(T) - \text{CASL}(T)
    \]
    This provides a clear indication of whether LPs are profiting or losing over the simulation period.
\end{itemize}

\section*{Sequencer Revenue Statistics}

\textbf{Motivation:}  
Sequencers earn revenue by collecting gas and priority fees from successful arbitrageurs. The size of these fees depends on the competition among arbitrageurs (i.e., how many bid for the same opportunity) and the value of the arbitrage opportunity (i.e., the difference between the true price and the onchain price). Understanding the sequencer’s revenue helps quantify the incentives for sequencers to facilitate fast transaction ordering and prioritize arbitrage transactions.

\textbf{Steps to Compute:}  
We will compute the following metrics to quantify sequencer revenue:

\begin{itemize}
    \item \textbf{Expected Revenue per Arbitrage (ERA)}: This will calculate the expected revenue for the sequencer from each arbitrage transaction, based on the value of the arbitrage opportunity. At each time step $t$, the revenue is:
    \[
    \text{ERA}(t) = g + \mathbb{E}[\text{Bid}(t)]
    \]
    where $g$ is the base gas fee and $\mathbb{E}[\text{Bid}(t)]$ is the expected priority fee from the arbitrageur with the winning bid. This allows us to assess how much revenue the sequencer is earning from each transaction.

    \item \textbf{Cumulative Sequencer Revenue (CSR)}: This will calculate the total revenue collected by the sequencer over the entire simulation:
    \[
    \text{CSR}(T) = \sum_{t=0}^{T} \text{ERA}(t)
    \]
    This captures the overall financial performance of the sequencer.

    \item \textbf{Revenue Distribution (RD)}: We will plot the distribution of sequencer revenues across all arbitrage transactions. By examining this distribution, we can see how frequently the sequencer earns higher or lower fees based on the size of arbitrage opportunities and competition among bidders.
\end{itemize}


\subsection{Parameter Choices}






==> old/old9-discussion-of-sim-result.tex <==
\section{Discussion}
This section examines how changes in key parameters—such as the number of arbitrageurs, gas fees, and liquidity depth—affect sequencer revenue and LP losses. We test the robustness of the model's predictions by varying these parameters.

\subsection{Effect of individual parameters}
\subsection{Effect of interactions}
